Field Trial of a Flexible Real-time Software-defined GPU-based Optical Receiver

We introduce a flexible, software-defined real-time multi-modulation format receiver implemented on an off-the-shelf general-purpose graphics processing unit (GPU). The flexible receiver is able to process 2 GBaud 2-, 4-, 8-, and 16-ary pulse-amplitude modulation (PAM) signals as well as 1 GBaud 4-, 16- and 64-ary quadrature amplitude modulation (QAM) signals, with the latter detected using a Kramers-Kronig (KK) coherent receiver. Experimental performance evaluation is shown for back-to-back. In addition, by using the JGN high speed R&D network testbed, performance is evaluated after transmission over 91 km field-deployed optical fiber and reconfigurable optical add-drop multiplexers (ROADMs).

==> sections/expsetup.tex <==
% %!TEX root = ../bare_jrnl.tex
% \section{Experimental setup using field trial network}
% \label{sec:expsetup}

% % \cref{fig:expsetup} shows a diagram of the experimental setup, including the field trial network. At the transmitter, the lightwave from a \SI{500}{kHz} linewidth \gls{ECL} centered at \SI{1542.92}{nm} is modulated using a single-polarization \gls{IQM}. Electrical driving signals for the \gls{IQM} are provided by a 2-channel \gls{AWG} operating at \SI{12}{Gs\per \second} amplified by RF-amplifiers, whilst bias-tees and voltage sources control the bias of the modulator arms.

% % \Gls{KK} \QAM{N} signals are modulated by operating the \gls{IQM} at the minimum optical output bias point, whilst the \gls{AWG} produces baseband 1~GBaud \QAM{N} signals with 1\% roll-off \gls{RRC} pulse shaping combined with a digitally-introduced carrier tone at a frequency of 0.547~GHz. The optimization of the tone power to produce the desired \gls{CSPR} is discussed in \cref{ssec:cspropt}. \PAM{N} signals are modulated by biasing one of the \gls{IQM}-arms to mid-point and driving it with a baseband 2~Gbaud 50\% roll-off \gls{RRC} pulse-shaped signal. 

% The signal launch power is set by an \gls{EDFA} followed by a \gls{VOA}. The transmission network consists of a bidirectional ring with 3 commercial \glspl{ROADM}. Two \glspl{ROADM} are installed in the same location in Koganei, Tokyo. The link between these \glspl{ROADM} is relatively short and its loss was set to \SI{16}{dB} using fixed attenuators. Both \glspl{ROADM} are connected to a commercial \gls{ROADM} in Otemachi, Tokyo by a \SI{45.5}{km}, 4-fiber link. The transmission loss, including optical distribution frames, is \SI{16.5}{dB}. 56\% of the fiber is installed in underground ducts and the remainder on areal paths and in the surface along railway tracks. The red line in \cref{fig:expsetup}) shows the signal path along the network, with a total transmission distance of \SI{91}{km}. Each \gls{ROADM} has two line sides, each consisting of \glspl{WSS} and optical amplifiers for add/drop and express connections. In addition, \glspl{ARRWG} were used for add and drop. \cref{fig:expsetup} shows a photograph of one of the commercial \glspl{ROADM}. 

% The receiver consists of an \gls{EDFA} pre-amplifier followed by a 0.04~nm \gls{BPF}. In addition, a noise-loading setup is included with an \gls{ASE} source and an \gls{OSA} through a 2$\times$2 coupler. A \gls{VOA} is used to control the power at the input of a \gls{PD} with a \SI{3}{dB} cut-off frequency of \SI{1}{GHz}. The electrical \gls{PD} output is directed to the \gls{ADC} for processing as described in sections \cref{sec:rxarch,sec:imdd,sec:kk}. Note that for back-to-back investigations, the output of the transmitter \gls{VOA} is routed via short patch cords via fixed attenuators \todo{[Was this really the case?]} to the receiver structure including noise-loading.
